The Landscape and Challenges of HPC Research and LLMs

Recently, language models (LMs), especially large language models (LLMs), have revolutionized the field of deep learning. Both encoder-decoder models and prompt-based techniques have shown immense potential for natural language processing and code-based tasks. Over the past several years, many research labs and institutions have invested heavily in high-performance computing, approaching or breaching exascale performance levels. In this paper, we posit that adapting and utilizing such language model-based techniques for tasks in high-performance computing (HPC) would be very beneficial. This study presents our reasoning behind the aforementioned position and highlights how existing ideas can be improved and adapted for HPC tasks.

==> sections/8-implementation.tex <==
\section{Implementation Strategies}

\subsection{Integrating LLMs into Existing HPC Workflows}

\subsection{Parallel Processing and Distributed Computing with LLMs}

\subsection{Optimizing LLMs for HPC Architecture}

\subsection{Scaling Up LLMs for Large-Scale HPC Applications}

\subsection{Datasets and Benchmarks}
